Pre-trained Molecular Language Models with Random Functional Group Masking

Recent advancements in computational chemistry have leveraged the power of trans-former-based language models, such as MoLFormer, pre-trained using a vast amount of simplified molecular-input line-entry system (SMILES) sequences, to understand and predict molecular properties and activities, a critical step in fields like drug discovery and materials science. To further improve performance, researchers have introduced graph neural networks with graph-based molecular representations, such as GEM, incorporating the topology, geometry, 2D or even 3D structures of molecules into pre-training. While most of molecular graphs in existing studies were automatically converted from SMILES sequences, it is to assume that transformer-based language models might be able to implicitly learn structure-aware representations from SMILES sequences. In this paper, we propose \ours{} -- a SMILES-based \underline{\em M}olecular \underline{\em L}anguage \underline{\em M}odel, which randomly masking SMILES subsequences corresponding to specific molecular \underline{\em F}unctional \underline{\em G}roups to incorporate structure information of atoms during the pre-training phase. This technique aims to compel the model to better infer molecular structures and properties, thus enhancing its predictive capabilities. Extensive experimental evaluations across 11 benchmark classification and regression tasks in the chemical domain demonstrate the robustness and superiority of \ours{}. Our findings reveal that \ours{} outperforms existing pre-training models, either based on SMILES or graphs, in 9 out of the 11 downstream tasks, ranking as a close second in the remaining ones.

==> table.tex <==
\begin{table*}[!t]
\centering
\caption{Comparison of fine-tuned \ours{} with existing supervised and pretrained/self-supervised baselines on multiple classification benchmarks.}
\scalebox{0.9}{
\begin{tabular}{cccccccc}
\toprule
& BBBP   & BACE   & ClinTox & Tox21  & SIDER  & HIV    & MUV    \\ \hline
No. molecules & 2,039 & 1,513 & 1,478 & 7,831 & 1,427 & 41,127 & 93,087 \\
No. prediction tasks & 1 & 1 & 2 & 12 & 27 & 1 & 17 \\
\hline
\multicolumn{8}{c}{Pre-trained models from existing literature}\\ \hline
MolCLR-gin                 & 0.9307 & 0.7873 & 0.8005  & 0.7644 & 0.5826 & 0.7768 & 0.7386 \\
MolCLR-gcn                 & 0.8432 & 0.7194 & 0.7997  & 0.7179 & 0.5353 & 0.7616 & 0.6701 \\
GROVER-base                & 0.9022 & 0.7700 & 0.6847  & 0.7187 & 0.5579 & 0.6950 & 0.6265 \\
GROVER-large               & 0.8861 & 0.7795 & 0.6082  & 0.7155 & 0.5283 & 0.6956 & 0.5132 \\
GEM                        & 0.9103 & 0.8603 & 0.8506  & 0.7791 & 0.6279 & 0.7500 & 0.7253 \\
Molformer                  & 0.9037 & 0.8275 & 0.9451  & 0.7734 & 0.5826 & 0.7630 & 0.7599 \\ \hline
\multicolumn{8}{c}{Transformer and RoBERTa models without pre-training}\\ \hline
Transformer (from scratch) & 0.8636 & 0.7728 & 0.7317  & 0.7461 & 0.5667 & 0.6991 & 0.6863 \\
RoBERTa (from scratch)     & 0.8711 & 0.7445 & 0.8858  & 0.7369 & 0.5285 & 0.5575 & 0.6674 \\ \hline
\multicolumn{8}{c}{RoBERTa models pre-trained by random subsequence masking}\\ \hline
RoBERTa (10M, rand. subseq) & 0.8572 & 0.8253 & 0.9284  & 0.7533 & 0.6111 & 0.7006 & 0.6234 \\
RoBERTa (20M, rand. subseq) & 0.9068 & 0.8135 & 0.9011 & 0.7635 & 0.5799 & 0.7477 & 0.6481 \\
RoBERTa (100M, rand. subseq) & 0.9048 & 0.8248 & 0.9167 & 0.7852 & 0.5860 & 0.7683 & 0.6909 \\ \hline
\multicolumn{8}{c}{Transformer and RoBERTa models pre-trained by \ours{}}\\ \hline
Transformer (10M)          & 0.8980 & 0.8044 & 0.9669  & 0.7765 & 0.5811 & 0.7633 & 0.6829 \\
Transformer (20M)          & 0.8976 & 0.8088 & 0.9436  & 0.7793 & 0.5992 & 0.7801 & 0.7185 \\
Transformer (100M)         & 0.9055 & 0.8040 & 0.9270  & 0.7893 & 0.5786 & 0.7690 & 0.6017 \\ %\hline
RoBERTa (10M)              & 0.8870 & 0.8265 & 0.9258  & 0.7545 & 0.6054 & 0.7106 & 0.6103 \\
RoBERTa (20M)              & 0.9378 & 0.8458 & 0.8919  & 0.7603 & 0.5908 & 0.7594 & 0.6428 \\
RoBERTa (100M)             & 0.9237 & 0.7981 & 0.9606  & 0.7896 & 0.6042 & 0.7807 & 0.7990 \\
\bottomrule
\end{tabular}
}
\label{exp:cls}
\end{table*}


\begin{table*}[!t]
\centering
\caption{Comparison of fine-tuned \ours{} with existing supervised and pretrained/self-supervised baselines on multiple regression benchmarks.}
\scalebox{1}{
\begin{tabular}{cccccc}
\toprule
& ESOL        & FreeSolv & Lipo   & QM7      & QM8    \\ \hline
No. molecules & 1,128 & 642 & 4,200 & 6,830 & 21,786 \\
No. prediction tasks & 1 & 1 & 1 & 1 & 12 \\
\hline
\multicolumn{6}{c}{Pre-trained models from existing literature}\\ \hline
MolCLR-gin                  & 1.4717      & 2.7116   & 0.7411 & 96.5469  & 0.0205 \\
MolCLR-gcn                  & 1.5074      & 2.7273   & 0.9033 & 93.5973  & 0.0235 \\
GROVER-base                 & 0.8813      & 1.5772   & 0.6664 & 101.2853 & 0.0228 \\
GROVER-large                & 0.8831      & 2.7143   & 0.7063 & 114.3004 & 0.0234 \\
GEM                         & 0.7614      & 2.4581   & 0.6861 & 65.0067  & 0.0179 \\
Molformer                   & 0.6613      & 4.4485   & 0.4457 & 69.0700  & 0.0177 \\ \hline
\multicolumn{6}{c}{Transformer and RoBERTa models without pre-training}\\ \hline
Transformer (from scratch)  & 0.9721      & 3.3689   & 0.9500 & 68.6214  & 0.0279 \\
RoBERTa  (from scratch)     & 0.9513      & 3.6014   & 0.9910 & 66.8488  & 0.0244 \\ \hline
\multicolumn{6}{c}{RoBERTa models pre-trained by random subsequence masking}\\ \hline
RoBERTa  (10M, subsequence) & 0.4909      & 4.4444   & 0.4515 & 68.4687  & 0.0219 \\
RoBERTa  (20M, subsequence) & 0.4596 & 3.1672 & 0.4560 & 70.1688 & 0.0207 \\
RoBERTa  (100M, subsequence) & 0.4301 & 2.4527 & 0.4430 & 76.6563 & 0.0232\\ \hline
\multicolumn{6}{c}{Transformer and RoBERTa models pre-trained by \ours{}}\\ \hline
Transformer (10M)           & 0.3432      & 5.5461   & 0.4919 & 67.7549  & 0.0221 \\
Transformer (20M)           & 0.4407      & 3.7525   & 0.4325 & 66.2175  & 0.0226 \\
Transformer (100M)          & 0.5135 & 3.2596   & 0.4272 & 69.3677  & 0.0212 \\ %\hline
RoBERTa (10M)               & 0.5707      & 1.7430   & 0.4892 & 66.9334  & 0.0212 \\
RoBERTa (20M)               & 0.6668      & 1.9143   & 0.6711 & 64.1665  & 0.0220 \\
RoBERTa (100M)              & 0.3901      & 3.0487   & 0.3984 & 74.8177  & 0.0202 \\
\bottomrule
\end{tabular}
}
\label{exp:reg}
\end{table*}
